Evolution of topics in central bank speech communication

This paper studies the content of central bank speech communication from 1997 through 2020 and asks the following questions: (i) What global topics do central banks talk about? (ii) How do these topics evolve over time? I turn to natural language processing, and more specifically Dynamic Topic Models, to answer these questions. The analysis consists of an aggregate study of nine major central banks and a case study of the Federal Reserve, which allows for region specific control variables. I show that: (i) Central banks address a broad range of topics. (ii) The topics are well captured by Dynamic Topic Models. (iii) The global topics exhibit strong and significant autoregressive properties not easily explained by financial control variables.

==> topics_table.tex <==
\scalebox{0.7}{
\begin{tabular}{a|b}\hline\hline
&Average \mathrm{P} (\%) in corpus\\
0: Supervision&3.17\\
1: Money&1.61\\
2: Financial stability&7.25\\
3: Payment&2.77\\
4: Euro area&2.63\\
5: Community&3.3\\
6: Financial system&2.56\\
7: Unemployment&1.61\\
8: Investor&5.33\\
9: Innovation&2.63\\
10: Liquidity&1.93\\
11: Model&4.37\\
12: Fiscal&5.51\\
13: Productivity&3.88\\
14: Trade&4.37\\
15: FOMC&2.14\\
16: Deflation&2.55\\
17: Australia&2.97\\
18: Canada&7.02\\
19: ECB&3.01\\
20: Euro area&4.54\\
21: Federal reserve&4.67\\
22: Japan economy&1.76\\
23: Japan&5.29\\
24: Norway&2.12\\
25: Riksbank&2.89\\
26: Residual&4.08\\
27: SNB&2.54\\
28: UK&1.53\\
Mean&3.45\\
Sum&100.0\\
\hline\hline
\end{tabular}
}

==> var_m_mod.tex <==
% In order to make the table nice after it has been outputted from Stata:
% 1. Add the following to the second header:
%\multicolumn{1}{c}{\shortstack{Model $\rightarrow$\\Lagged variables (1 lag) $\downarrow$}}
% 2. Change the tabular to:
%       \begin{tabular}{l a b a b a b a b a b a}
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l a b a b a b a b a b a b a b a b a b a b a b a b a b a b a}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}&\multicolumn{1}{c}{(11)}&\multicolumn{1}{c}{(12)}&\multicolumn{1}{c}{(13)}&\multicolumn{1}{c}{(14)}&\multicolumn{1}{c}{(15)}&\multicolumn{1}{c}{(16)}&\multicolumn{1}{c}{(17)}\\
\multicolumn{1}{c}{\shortstack{Model $\rightarrow$\\Lagged variables (1 lag) $\downarrow$}}  &\multicolumn{1}{c}{Regulation}&\multicolumn{1}{c}{Money}&\multicolumn{1}{c}{\shortstack{Financial\\stability}}&\multicolumn{1}{c}{Payment}&\multicolumn{1}{c}{\shortstack{Euro\\area}}&\multicolumn{1}{c}{Community}&\multicolumn{1}{c}{\shortstack{Financial\\system}}&\multicolumn{1}{c}{Unemployment}&\multicolumn{1}{c}{Investor}&\multicolumn{1}{c}{Innovation}&\multicolumn{1}{c}{Liquidity}&\multicolumn{1}{c}{Model}&\multicolumn{1}{c}{Fiscal}&\multicolumn{1}{c}{Productivity}&\multicolumn{1}{c}{Trade}&\multicolumn{1}{c}{FOMC}&\multicolumn{1}{c}{Deflation}\\
\hline
Regulation  &      0.0271         &     -0.0653\sym{*}  &    -0.00980         &     -0.0142         &      0.0208         &      0.0379         &      -0.119         &     -0.0627         &     -0.0324         &    -0.00438         &      -0.150\sym{**} &     0.00265         &     0.00929         &       0.134         &       0.129         &     -0.0641         &     -0.0612         \\
            &      (0.39)         &     (-2.18)         &     (-0.17)         &     (-0.21)         &      (0.32)         &      (0.65)         &     (-1.64)         &     (-1.19)         &     (-0.78)         &     (-0.09)         &     (-3.10)         &      (0.04)         &      (0.12)         &      (1.92)         &      (1.46)         &     (-1.24)         &     (-1.40)         \\
[1em]
Money       &     -0.0274         &       0.193\sym{*}  &     -0.0698         &       0.150         &     -0.0167         &      -0.134         &      0.0102         &       0.141         &     -0.0144         &      0.0605         &      -0.231         &      -0.245         &       0.159         &      0.0559         &     -0.0816         &      -0.223         &      0.0338         \\
            &     (-0.31)         &      (2.45)         &     (-0.75)         &      (0.78)         &     (-0.13)         &     (-1.49)         &      (0.05)         &      (1.08)         &     (-0.15)         &      (0.88)         &     (-1.50)         &     (-1.91)         &      (1.13)         &      (0.37)         &     (-0.62)         &     (-1.85)         &      (0.36)         \\
[1em]
\shortstack{Financial\\stability}&     -0.0244         &     -0.0242         &       0.201\sym{**} &      0.0356         &     -0.0589         &      0.0529         &       0.125         &     -0.0725         &      0.0168         &      0.0257         &      0.0990         &       0.116         &      0.0767         &      0.0645         &      0.0905         &      0.0344         &     -0.0253         \\
            &     (-0.42)         &     (-0.92)         &      (2.67)         &      (0.69)         &     (-1.13)         &      (0.80)         &      (1.60)         &     (-1.49)         &      (0.32)         &      (0.72)         &      (1.38)         &      (1.92)         &      (0.98)         &      (0.63)         &      (1.01)         &      (0.50)         &     (-0.47)         \\
[1em]
Payment     &     -0.0730         &      0.0289         &   -0.000268         &       0.164\sym{*}  &     -0.0277         &     0.00335         &     0.00126         &     -0.0334         &       0.199\sym{**} &      0.0851\sym{*}  &       0.148\sym{*}  &      0.0426         &     -0.0139         &      -0.100         &      0.0345         &      0.0847         &       0.123         \\
            &     (-1.25)         &      (0.91)         &     (-0.01)         &      (2.29)         &     (-0.33)         &      (0.05)         &      (0.01)         &     (-0.69)         &      (3.15)         &      (2.09)         &      (2.44)         &      (0.65)         &     (-0.16)         &     (-1.39)         &      (0.37)         &      (1.35)         &      (1.94)         \\
[1em]
\shortstack{Euro\\area}&       0.165\sym{***}&    -0.00476         &     0.00357         &     -0.0310         &       0.590\sym{***}&      0.0234         &    -0.00195         &      -0.129\sym{***}&      0.0104         &      0.0165         &    -0.00897         &     -0.0518         &     -0.0174         &     -0.0979\sym{*}  &      -0.107\sym{**} &       0.129\sym{**} &       0.160\sym{***}\\
            &      (3.76)         &     (-0.19)         &      (0.08)         &     (-0.58)         &      (6.72)         &      (0.48)         &     (-0.04)         &     (-3.82)         &      (0.30)         &      (0.54)         &     (-0.20)         &     (-1.16)         &     (-0.20)         &     (-2.58)         &     (-2.65)         &      (2.91)         &      (3.77)         \\
[1em]
Community   &      0.0451         &    -0.00437         &      0.0754         &    0.000424         &      0.0422         &       0.111\sym{*}  &      0.0525         &     -0.0738         &      0.0817         &      0.0214         &      0.0624         &      0.0742         &       0.188\sym{*}  &      -0.107         &     -0.0862         &      0.0196         &      0.0877\sym{*}  \\
            &      (0.80)         &     (-0.15)         &      (1.16)         &      (0.01)         &      (0.66)         &      (1.98)         &      (0.85)         &     (-1.38)         &      (1.97)         &      (0.60)         &      (1.03)         &      (1.30)         &      (2.17)         &     (-1.90)         &     (-1.24)         &      (0.43)         &      (2.16)         \\
[1em]
\shortstack{Financial\\system}&    -0.00708         &     -0.0549         &       0.206\sym{***}&     -0.0583         &     0.00219         &     -0.0177         &       0.403\sym{***}&      0.0466         &     -0.0525         &     -0.0858\sym{*}  &      0.0239         &     -0.0477         &       0.212\sym{***}&      -0.190\sym{*}  &      0.0167         &     -0.0920\sym{*}  &     -0.0215         \\
            &     (-0.19)         &     (-1.69)         &      (3.47)         &     (-1.44)         &      (0.06)         &     (-0.31)         &      (6.96)         &      (0.88)         &     (-0.98)         &     (-2.33)         &      (0.43)         &     (-0.87)         &      (3.34)         &     (-2.50)         &      (0.22)         &     (-2.08)         &     (-0.60)         \\
[1em]
Unemployment&       0.108         &      0.0199         &      0.0538         &      0.0887         &      -0.151         &     -0.0288         &      0.0297         &      0.0599         &      0.0506         &      0.0595         &      -0.116         &      0.0431         &     -0.0734         &       0.325\sym{**} &     0.00263         &    -0.00790         &      -0.102\sym{*}  \\
            &      (1.29)         &      (0.45)         &      (0.59)         &      (1.22)         &     (-1.96)         &     (-0.43)         &      (0.24)         &      (0.81)         &      (0.99)         &      (1.10)         &     (-1.81)         &      (0.49)         &     (-0.87)         &      (2.65)         &      (0.03)         &     (-0.11)         &     (-2.05)         \\
[1em]
Investor    &      0.0197         &     -0.0663         &      -0.115         &       0.181\sym{*}  &     -0.0192         &       0.158         &      -0.300\sym{***}&      0.0281         &      0.0197         &     0.00756         &      0.0966         &      -0.177\sym{**} &      0.0304         &       0.127         &     -0.0611         &      0.0988         &    -0.00333         \\
            &      (0.30)         &     (-1.88)         &     (-1.58)         &      (2.17)         &     (-0.19)         &      (1.70)         &     (-3.89)         &      (0.47)         &      (0.24)         &      (0.15)         &      (0.53)         &     (-2.62)         &      (0.21)         &      (1.36)         &     (-0.85)         &      (1.35)         &     (-0.04)         \\
[1em]
Innovation  &      0.0671         &     -0.0819         &       0.143         &     -0.0102         &       0.128         &     -0.0125         &      0.0781         &     -0.0556         &      0.0123         &      0.0429         &      -0.240\sym{*}  &     -0.0428         &    -0.00327         &       0.125         &       0.108         &      -0.111         &     -0.0146         \\
            &      (0.75)         &     (-1.76)         &      (1.84)         &     (-0.11)         &      (1.34)         &     (-0.14)         &      (0.62)         &     (-0.70)         &      (0.18)         &      (0.70)         &     (-2.51)         &     (-0.45)         &     (-0.03)         &      (0.93)         &      (0.96)         &     (-1.24)         &     (-0.22)         \\
[1em]
Liquidity   &     -0.0795\sym{*}  &    -0.00887         &      0.0561         &     -0.0155         &     -0.0371         &       0.196\sym{***}&       0.141         &      -0.130\sym{***}&     -0.0137         &     -0.0493         &       0.593\sym{***}&     -0.0313         &      -0.202\sym{**} &     -0.0670         &     -0.0555         &     -0.0453         &    -0.00515         \\
            &     (-2.27)         &     (-0.34)         &      (1.08)         &     (-0.31)         &     (-0.68)         &      (3.44)         &      (1.96)         &     (-3.67)         &     (-0.35)         &     (-1.93)         &      (8.71)         &     (-0.60)         &     (-3.08)         &     (-1.27)         &     (-1.12)         &     (-1.13)         &     (-0.13)         \\
[1em]
Model       &      0.0630         &     -0.0533         &       0.137         &      -0.159\sym{**} &      0.0252         &      0.0443         &       0.152         &     -0.0696         &     -0.0150         &      0.0496         &      0.0141         &      0.0677         &    0.000415         &      -0.105         &      0.0688         &     -0.0877         &     -0.0613         \\
            &      (1.22)         &     (-1.39)         &      (1.97)         &     (-2.92)         &      (0.42)         &      (0.74)         &      (1.79)         &     (-1.26)         &     (-0.34)         &      (1.16)         &      (0.22)         &      (0.95)         &      (0.01)         &     (-1.13)         &      (0.91)         &     (-1.34)         &     (-1.24)         \\
[1em]
Fiscal      &    -0.00349         &     -0.0355         &      0.0700         &      -0.111\sym{**} &     -0.0251         &       0.121\sym{*}  &      0.0505         &     -0.0194         &     -0.0342         &      0.0136         &      0.0843         &      0.0144         &       0.348\sym{***}&     0.00220         &     0.00523         &      0.0261         &     -0.0277         \\
            &     (-0.09)         &     (-1.67)         &      (1.60)         &     (-2.72)         &     (-0.42)         &      (2.22)         &      (0.97)         &     (-0.64)         &     (-0.97)         &      (0.50)         &      (0.92)         &      (0.29)         &      (4.71)         &      (0.05)         &      (0.14)         &      (0.60)         &     (-0.63)         \\
[1em]
Productivity&     -0.0533         &     -0.0233         &      0.0390         &     -0.0534         &     -0.0401         &     -0.0633         &      0.0271         &       0.109\sym{**} &    -0.00851         &      0.0526         &    -0.00738         &      0.0198         &     -0.0775         &       0.200\sym{**} &      0.0384         &     -0.0192         &     -0.0450         \\
            &     (-0.89)         &     (-0.91)         &      (0.79)         &     (-1.17)         &     (-0.93)         &     (-1.54)         &      (0.41)         &      (2.60)         &     (-0.24)         &      (1.43)         &     (-0.17)         &      (0.34)         &     (-1.46)         &      (2.78)         &      (0.66)         &     (-0.34)         &     (-1.40)         \\
[1em]
Trade       &     -0.0301         &     -0.0146         &    0.000446         &    -0.00318         &      -0.108\sym{*}  &     0.00557         &     -0.0452         &      0.0179         &      0.0231         &     -0.0383         &      -0.136\sym{**} &      0.0189         &      -0.126\sym{*}  &       0.109         &       0.310\sym{***}&     -0.0321         &      -0.118\sym{***}\\
            &     (-0.49)         &     (-0.70)         &      (0.01)         &     (-0.07)         &     (-2.28)         &      (0.11)         &     (-0.64)         &      (0.29)         &      (0.52)         &     (-1.11)         &     (-3.27)         &      (0.29)         &     (-2.18)         &      (1.17)         &      (4.14)         &     (-0.49)         &     (-3.34)         \\
[1em]
FOMC        &    -0.00252         &      0.0279         &      0.0338         &       0.149\sym{*}  &       0.145         &      0.0751         &    -0.00158         &    -0.00206         &       0.117\sym{*}  &      0.0221         &      -0.149         &      0.0386         &      0.0733         &      -0.151         &      0.0360         &      0.0331         &      0.0565         \\
            &     (-0.05)         &      (0.91)         &      (0.50)         &      (2.29)         &      (1.62)         &      (1.06)         &     (-0.02)         &     (-0.04)         &      (2.07)         &      (0.46)         &     (-1.86)         &      (0.51)         &      (0.88)         &     (-1.82)         &      (0.44)         &      (0.48)         &      (0.81)         \\
[1em]
Deflation   &      0.0946         &      0.0273         &     -0.0120         &       0.239\sym{***}&       0.113         &     -0.0672         &     -0.0202         &      -0.159\sym{***}&       0.240\sym{***}&     -0.0256         &     -0.0449         &     -0.0709         &       0.179         &     -0.0460         &      -0.171\sym{**} &      0.0557         &       0.406\sym{***}\\
            &      (1.53)         &      (0.79)         &     (-0.19)         &      (3.34)         &      (1.23)         &     (-0.93)         &     (-0.26)         &     (-3.77)         &      (3.73)         &     (-0.64)         &     (-0.60)         &     (-1.12)         &      (1.68)         &     (-0.64)         &     (-2.83)         &      (0.81)         &      (4.68)         \\
[1em]
Constants   &      0.0190         &      0.0214\sym{**} &    0.000136         &      0.0195         &      0.0160         &     0.00949         &      0.0172         &      0.0490\sym{***}&     0.00408         &      0.0194\sym{**} &      0.0264\sym{*}  &      0.0453\sym{***}&      0.0133         &      0.0368\sym{*}  &      0.0215         &      0.0396\sym{**} &      0.0202\sym{*}  \\
            &      (1.74)         &      (2.61)         &      (0.01)         &      (1.79)         &      (1.59)         &      (1.06)         &      (1.37)         &      (5.03)         &      (0.54)         &      (2.70)         &      (2.30)         &      (4.33)         &      (1.04)         &      (2.42)         &      (1.87)         &      (3.22)         &      (2.55)         \\
\hline
\(N\)       &         287         &         287         &         287         &         287         &         287         &         287         &         287         &         287         &         287         &         287         &         287         &         287         &         287         &         287         &         287         &         287         &         287         \\
\hline\hline
\multicolumn{18}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{18}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> var_q_control_4_mod.tex <==
% In order to make the table nice after it has been outputted from Stata:
% 1. Add the following to the second header:
%\multicolumn{1}{c}{\shortstack{Model $\rightarrow$\\Lagged variables (1 lag) $\downarrow$}}
% 2. Change the tabular to:
%       \begin{tabular}{l a b a b a b a b a b a}
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l a b a b a b a b a b a b a b a b a b a b a b a b a b a b a}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\multicolumn{1}{c}{\shortstack{Model $\rightarrow$\\Lagged variables (1 lag) $\downarrow$}}
            &\multicolumn{1}{c}{Housing}&\multicolumn{1}{c}{Regulation}&\multicolumn{1}{c}{\shortstack{Financial\\markets}}&\multicolumn{1}{c}{Trade}&\multicolumn{1}{c}{Purchase}\\
\hline
Housing     &       0.795\sym{***}&       0.127         &       0.291         &     -0.0715         &       0.423\sym{***}\\
            &      (7.88)         &      (0.88)         &      (1.93)         &     (-0.72)         &      (4.64)         \\
[1em]
Regulation  &      -0.120         &       0.431\sym{**} &       0.146         &      -0.275\sym{**} &       0.152\sym{*}  \\
            &     (-1.09)         &      (3.39)         &      (1.06)         &     (-3.23)         &      (2.11)         \\
[1em]
\shortstack{Financial\\markets}&      0.0884         &     -0.0978         &      0.0887         &       0.256\sym{*}  &     -0.0472         \\
            &      (0.68)         &     (-0.63)         &      (0.61)         &      (2.18)         &     (-0.49)         \\
[1em]
Trade       &      0.0425         &      -0.121         &      0.0881         &      0.0138         &       0.112         \\
            &      (0.40)         &     (-0.93)         &      (0.59)         &      (0.14)         &      (1.11)         \\
[1em]
Purchase    &       0.123         &       0.408\sym{*}  &       0.349\sym{**} &     -0.0278         &       0.267\sym{**} \\
            &      (1.56)         &      (2.37)         &      (2.77)         &     (-0.30)         &      (2.94)         \\
[1em]
Constants   &     -0.0202         &      0.0862\sym{*}  &      0.0989\sym{**} &       0.105\sym{***}&     -0.0415         \\
            &     (-0.85)         &      (2.04)         &      (3.30)         &      (4.03)         &     (-1.79)         \\
\hline
\(N\)       &          92         &          92         &          92         &          92         &          92         \\
\hline\hline
\multicolumn{6}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{6}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> var_q_control_mod.tex <==
% In order to make the table nice after it has been outputted from Stata:
% 1. Add the following to the second header:
%\multicolumn{1}{c}{\shortstack{Model $\rightarrow$\\Lagged variables (1 lag) $\downarrow$}}
% 2. Change the tabular to:
%       \begin{tabular}{l a b a b a b a b a b a}
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l a b a b a b a b a b a b a b a b a b a b a b a b a b a b a}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
\multicolumn{1}{c}{\shortstack{Model $\rightarrow$\\Lagged variables (1 lag) $\downarrow$}}
            &\multicolumn{1}{c}{Housing}&\multicolumn{1}{c}{Regulation}&\multicolumn{1}{c}{\shortstack{Financial\\markets}}&\multicolumn{1}{c}{Trade}&\multicolumn{1}{c}{Purchase}&\multicolumn{1}{c}{CPI}&\multicolumn{1}{c}{\shortstack{1 year\\treasury}}&\multicolumn{1}{c}{\shortstack{SP500\\returns}}&\multicolumn{1}{c}{\shortstack{SP500\\index}}&\multicolumn{1}{c}{VIX}\\
\hline
Housing     &       0.764\sym{***}&     -0.0443         &       0.271\sym{*}  &     -0.0800         &       0.359\sym{***}&   -1.99e-17         &   -1.98e-17         &    2.90e-17         &    1.09e-12         &    1.98e-15         \\
            &      (7.44)         &     (-0.34)         &      (2.23)         &     (-0.96)         &      (5.44)         &     (-1.65)         &     (-1.65)         &      (1.21)         &      (0.59)         &      (0.11)         \\
[1em]
Regulation  &     -0.0378         &       0.350\sym{**} &      0.0477         &      -0.215\sym{*}  &       0.238\sym{***}&    5.73e-18         &    9.47e-19         &   -1.29e-17         &    2.16e-12         &   -2.39e-14         \\
            &     (-0.49)         &      (3.24)         &      (0.53)         &     (-2.51)         &      (3.73)         &      (0.81)         &      (0.11)         &     (-0.85)         &      (1.23)         &     (-1.74)         \\
[1em]
\shortstack{Financial\\markets}&      0.0513         &       0.142         &       0.168         &       0.202         &     -0.0517         &    6.20e-19         &   -9.53e-19         &    2.20e-17         &   -2.54e-12         &    4.40e-15         \\
            &      (0.45)         &      (0.83)         &      (1.39)         &      (1.91)         &     (-0.66)         &      (0.06)         &     (-0.10)         &      (1.00)         &     (-1.12)         &      (0.31)         \\
[1em]
Trade       &      0.0773         &      -0.115         &       0.146         &      0.0646         &       0.102         &    1.54e-19         &    8.39e-18         &   -4.46e-17         &    8.25e-13         &    3.35e-15         \\
            &      (0.76)         &     (-0.92)         &      (1.14)         &      (0.66)         &      (1.37)         &      (0.01)         &      (0.82)         &     (-1.80)         &      (0.38)         &      (0.24)         \\
[1em]
Purchase    &      0.0113         &       0.334\sym{*}  &       0.289\sym{*}  &      -0.107         &       0.363\sym{***}&    3.83e-18         &    2.81e-17\sym{*}  &   -4.58e-17\sym{**} &    2.67e-12         &    4.46e-15         \\
            &      (0.10)         &      (2.09)         &      (2.64)         &     (-1.23)         &      (3.90)         &      (0.46)         &      (2.41)         &     (-2.66)         &      (1.13)         &      (0.19)         \\
[1em]
CPI         &      -0.630         &      -0.361         &      -0.825         &      0.0414         &      -1.692\sym{***}&           1\sym{***}&    3.79e-17         &    2.40e-16         &    9.77e-13         &   -2.65e-14         \\
            &     (-0.98)         &     (-0.63)         &     (-1.66)         &      (0.09)         &     (-4.37)         &  (1.37e+16)         &      (0.87)         &      (1.23)         &      (0.09)         &     (-0.37)         \\
[1em]
\shortstack{1 year\\treasury}&       0.861         &       0.641         &      -0.623         &      -0.752         &      -0.472         &   -7.02e-17         &       1.000\sym{***}&    4.36e-16\sym{**} &    2.23e-11         &    8.28e-14         \\
            &      (1.05)         &      (0.60)         &     (-0.69)         &     (-1.18)         &     (-0.71)         &     (-0.68)         &  (9.68e+15)         &      (3.28)         &      (1.13)         &      (0.67)         \\
[1em]
\shortstack{SP500\\returns}&       0.164         &      -1.255         &       0.306         &      -0.367         &     -0.0251         &    3.76e-16\sym{**} &   -7.68e-17         &       1.000\sym{***}&   -2.67e-11         &    4.09e-13\sym{***}\\
            &      (0.24)         &     (-1.59)         &      (0.51)         &     (-0.70)         &     (-0.04)         &      (3.17)         &     (-1.23)         &  (4.67e+15)         &     (-1.50)         &      (3.65)         \\
[1em]
\shortstack{SP500\\index}&  -0.0000467         &  -0.0000965         &  -0.0000362         &   0.0000101         &  -0.0000451         &    5.70e-22         &   -3.22e-20\sym{***}&   -1.51e-20         &       1.000\sym{***}&    2.47e-17\sym{**} \\
            &     (-0.81)         &     (-1.38)         &     (-0.58)         &      (0.22)         &     (-1.03)         &      (0.08)         &     (-3.88)         &     (-1.27)         &  (4.12e+14)         &      (2.81)         \\
[1em]
VIX         &   -0.000148         &    0.000823         &   -0.000505         &    0.000566         &   -0.000243         &   -3.82e-19\sym{**} &    1.08e-19         &    8.71e-19\sym{***}&    1.06e-14         &       1.000\sym{***}\\
            &     (-0.16)         &      (0.76)         &     (-0.61)         &      (0.85)         &     (-0.33)         &     (-2.85)         &      (1.28)         &      (3.69)         &      (0.46)         &  (7.01e+15)         \\
[1em]
CPI         &      -0.608         &     -0.0465         &       0.839         &      -0.218         &      -0.540         &    8.36e-17         &    1.53e-17         &   -1.27e-16         &   -5.50e-12         &    5.10e-15         \\
            &     (-1.42)         &     (-0.07)         &      (1.59)         &     (-0.55)         &     (-1.53)         &      (1.71)         &      (0.32)         &     (-1.54)         &     (-0.51)         &      (0.05)         \\
[1em]
\shortstack{1 year\\treasury}&      -0.340         &      -1.596         &       1.371         &       0.883         &     -0.0189         &   -5.77e-17         &    2.59e-16\sym{*}  &   -3.81e-16\sym{*}  &   -4.84e-12         &   -3.90e-15         \\
            &     (-0.52)         &     (-1.17)         &      (1.38)         &      (1.08)         &     (-0.02)         &     (-0.59)         &      (2.30)         &     (-2.15)         &     (-0.28)         &     (-0.03)         \\
[1em]
\shortstack{SP500\\returns}&      -0.407         &       0.316         &      -0.598         &      -0.672         &       0.619         &   -2.00e-16\sym{**} &   -1.20e-16         &   -2.24e-16         &   -1.07e-11         &   -6.72e-13\sym{***}\\
            &     (-0.67)         &      (0.39)         &     (-1.04)         &     (-1.05)         &      (1.32)         &     (-2.98)         &     (-1.32)         &     (-1.75)         &     (-0.63)         &     (-3.63)         \\
[1em]
\shortstack{SP500\\index}&   0.0000471         &   0.0000814         &   0.0000352         &  -0.0000272         &   0.0000707         &   -5.09e-22         &    3.24e-20\sym{***}&    1.52e-20         &    9.85e-15\sym{***}&   -2.60e-17\sym{**} \\
            &      (0.80)         &      (1.18)         &      (0.55)         &     (-0.57)         &      (1.57)         &     (-0.07)         &      (3.84)         &      (1.22)         &      (3.82)         &     (-2.85)         \\
[1em]
VIX         &    0.000522         &   -0.000436         &   0.0000186         &  -0.0000305         &    0.000549         &    2.73e-19\sym{**} &    1.70e-20         &    2.79e-19         &    7.07e-16         &    9.67e-16\sym{***}\\
            &      (0.57)         &     (-0.41)         &      (0.02)         &     (-0.04)         &      (0.67)         &      (2.97)         &      (0.16)         &      (1.64)         &      (0.03)         &      (3.99)         \\
[1em]
Constants   &     0.00391         &      0.0731\sym{**} &      0.0458\sym{*}  &      0.0938\sym{***}&     -0.0461\sym{*}  &   -2.60e-18         &    8.67e-19         &   -6.94e-18\sym{*}  &   -2.27e-13         &   -3.55e-15         \\
            &      (0.19)         &      (2.81)         &      (2.21)         &      (3.89)         &     (-2.22)         &     (-1.22)         &      (0.55)         &     (-2.08)         &     (-0.48)         &     (-1.50)         \\
\hline
\(N\)       &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> var_q_mod.tex <==
% In order to make the table nice after it has been outputted from Stata:
% 1. Add the following to the second header:
%\multicolumn{1}{c}{\shortstack{Model $\rightarrow$\\Lagged variables (1 lag) $\downarrow$}}
% 2. Change the tabular to:
%       \begin{tabular}{l a b a b a b a b a b a}
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l a b a b a b a b a b a b a b a b a}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}&\multicolumn{1}{c}{(11)}&\multicolumn{1}{c}{(12)}&\multicolumn{1}{c}{(13)}&\multicolumn{1}{c}{(14)}&\multicolumn{1}{c}{(15)}&\multicolumn{1}{c}{(16)}&\multicolumn{1}{c}{(17)}\\
\multicolumn{1}{c}{\shortstack{Model $\rightarrow$\\Lagged variables (1 lag) $\downarrow$}}            &\multicolumn{1}{c}{Regulation}&\multicolumn{1}{c}{Money}&\multicolumn{1}{c}{\shortstack{Financial\\stability}}&\multicolumn{1}{c}{Payment}&\multicolumn{1}{c}{\shortstack{Euro\\area}}&\multicolumn{1}{c}{Community}&\multicolumn{1}{c}{\shortstack{Financial\\system}}&\multicolumn{1}{c}{Unemployment}&\multicolumn{1}{c}{Investor}&\multicolumn{1}{c}{Innovation}&\multicolumn{1}{c}{Liquidity}&\multicolumn{1}{c}{Model}&\multicolumn{1}{c}{Fiscal}&\multicolumn{1}{c}{Productivity}&\multicolumn{1}{c}{Trade}&\multicolumn{1}{c}{FOMC}&\multicolumn{1}{c}{Deflation}\\
\hline
Regulation  &    -0.00353         &     -0.0592         &      -0.189         &     -0.0749         &      0.0337         &     -0.0623         &     -0.0415         &     -0.0940         &     0.00202         &     -0.0480         &      -0.277         &     -0.0218         &       0.168         &      0.0719         &       0.338         &       0.199\sym{*}  &     -0.0299         \\
            &     (-0.03)         &     (-1.41)         &     (-1.55)         &     (-0.73)         &      (0.40)         &     (-0.68)         &     (-0.33)         &     (-0.95)         &      (0.03)         &     (-0.74)         &     (-1.85)         &     (-0.21)         &      (1.27)         &      (0.51)         &      (1.88)         &      (2.16)         &     (-0.47)         \\
[1em]
Money       &      -0.479         &       0.177         &     -0.0537         &      -0.172         &       0.209         &       0.204         &       0.375         &       0.274         &      0.0255         &     -0.0383         &       0.706         &      -0.338         &       0.451         &      -0.268         &      -0.294         &      -0.157         &      -0.396\sym{**} \\
            &     (-1.68)         &      (1.20)         &     (-0.22)         &     (-0.63)         &      (0.71)         &      (0.83)         &      (1.57)         &      (1.13)         &      (0.12)         &     (-0.22)         &      (1.21)         &     (-1.50)         &      (1.34)         &     (-0.71)         &     (-0.94)         &     (-0.75)         &     (-2.71)         \\
[1em]
\shortstack{Financial\\stability}&      -0.211         &    -0.00907         &       0.188         &     -0.0671         &       0.242\sym{*}  &      0.0374         &      0.0673         &      -0.151\sym{*}  &      -0.105         &     0.00572         &       0.175         &       0.182         &       0.381\sym{**} &      -0.192         &     -0.0484         &     -0.0614         &     -0.0178         \\
            &     (-1.92)         &     (-0.25)         &      (1.75)         &     (-0.83)         &      (2.43)         &      (0.47)         &      (0.58)         &     (-2.20)         &     (-1.78)         &      (0.09)         &      (1.11)         &      (1.90)         &      (3.13)         &     (-1.38)         &     (-0.37)         &     (-0.62)         &     (-0.36)         \\
[1em]
Payment     &       0.321\sym{*}  &       0.121         &      0.0742         &       0.197         &     -0.0644         &      0.0595         &       0.245         &      -0.128         &       0.185\sym{*}  &      0.0625         &      0.0116         &      -0.170         &      0.0590         &      -0.205         &      0.0432         &      0.0189         &      0.0708         \\
            &      (2.63)         &      (1.73)         &      (0.74)         &      (1.35)         &     (-0.51)         &      (0.37)         &      (1.84)         &     (-1.53)         &      (2.27)         &      (0.84)         &      (0.09)         &     (-1.45)         &      (0.43)         &     (-1.30)         &      (0.33)         &      (0.18)         &      (0.90)         \\
[1em]
\shortstack{Euro\\area}&       0.247\sym{**} &      0.0132         &      0.0288         &     -0.0589         &       0.737\sym{***}&     -0.0421         &     -0.0746         &      -0.196\sym{***}&    -0.00311         &     -0.0196         &     -0.0981         &     -0.0485         &       0.110         &     -0.0412         &      -0.133         &       0.164\sym{*}  &       0.133\sym{**} \\
            &      (3.22)         &      (0.56)         &      (0.45)         &     (-0.88)         &      (6.91)         &     (-0.59)         &     (-1.20)         &     (-4.34)         &     (-0.06)         &     (-0.55)         &     (-0.81)         &     (-0.76)         &      (1.06)         &     (-0.59)         &     (-1.95)         &      (2.50)         &      (3.25)         \\
[1em]
Community   &      0.0708         &     -0.0423         &       0.285\sym{*}  &     -0.0182         &     -0.0478         &       0.370\sym{*}  &     -0.0220         &      -0.131         &      0.0173         &     0.00863         &      0.0871         &      0.0806         &       0.202         &      -0.425\sym{**} &      -0.225         &      0.0431         &      -0.128\sym{*}  \\
            &      (0.74)         &     (-0.86)         &      (2.10)         &     (-0.19)         &     (-0.36)         &      (2.27)         &     (-0.17)         &     (-1.56)         &      (0.20)         &      (0.14)         &      (0.74)         &      (0.76)         &      (1.65)         &     (-3.38)         &     (-1.81)         &      (0.58)         &     (-2.07)         \\
[1em]
\shortstack{Financial\\system}&     -0.0553         &     -0.0172         &       0.193\sym{*}  &     -0.0187         &     -0.0611         &      -0.173\sym{*}  &       0.580\sym{***}&    0.000959         &     -0.0325         &     -0.0748         &     -0.0608         &       0.128         &       0.111         &     -0.0459         &      0.0913         &       0.111         &     0.00786         \\
            &     (-0.56)         &     (-0.63)         &      (2.50)         &     (-0.32)         &     (-1.09)         &     (-2.60)         &      (6.57)         &      (0.01)         &     (-0.64)         &     (-1.76)         &     (-0.38)         &      (1.71)         &      (1.60)         &     (-0.33)         &      (0.98)         &      (1.24)         &      (0.22)         \\
[1em]
Unemployment&       0.160         &      0.0665         &     -0.0489         &      0.0941         &      -0.188         &      -0.215         &      -0.418\sym{*}  &      0.0861         &      0.0457         &    -0.00926         &      -0.297         &      0.0541         &      0.0294         &       0.612\sym{*}  &      -0.121         &       0.249         &     -0.0970         \\
            &      (0.75)         &      (0.81)         &     (-0.35)         &      (0.50)         &     (-1.35)         &     (-1.52)         &     (-2.05)         &      (0.67)         &      (0.43)         &     (-0.09)         &     (-1.71)         &      (0.39)         &      (0.16)         &      (2.29)         &     (-0.67)         &      (1.35)         &     (-1.10)         \\
[1em]
Investor    &      -0.354\sym{*}  &     -0.0421         &      -0.296\sym{*}  &       0.408\sym{*}  &      0.0947         &      0.0771         &      -0.316\sym{*}  &      -0.224\sym{*}  &       0.214         &      -0.121         &       0.332         &      -0.180         &       0.143         &       0.178         &      -0.142         &       0.369\sym{*}  &       0.268\sym{*}  \\
            &     (-2.34)         &     (-0.40)         &     (-2.06)         &      (2.36)         &      (0.55)         &      (0.34)         &     (-2.25)         &     (-2.34)         &      (1.68)         &     (-1.19)         &      (1.14)         &     (-1.03)         &      (0.80)         &      (0.79)         &     (-0.75)         &      (2.61)         &      (2.43)         \\
[1em]
Innovation  &      -0.402         &     -0.0204         &     -0.0149         &       0.106         &      -0.151         &     -0.0951         &      -0.464\sym{*}  &       0.120         &       0.133         &       0.331\sym{*}  &      -0.492         &       0.568\sym{***}&      -0.340         &       1.081\sym{***}&       0.345         &       0.443\sym{*}  &     -0.0780         \\
            &     (-1.64)         &     (-0.25)         &     (-0.08)         &      (0.46)         &     (-0.80)         &     (-0.59)         &     (-2.00)         &      (0.84)         &      (0.79)         &      (2.54)         &     (-1.75)         &      (3.58)         &     (-1.86)         &      (3.77)         &      (1.23)         &      (2.38)         &     (-0.73)         \\
[1em]
Liquidity   &     -0.0752         &    -0.00537         &     -0.0256         &      0.0329         &      -0.116         &       0.198\sym{*}  &      0.0814         &      -0.127         &      0.0457         &     -0.0531         &       0.550\sym{***}&     -0.0996         &      -0.164\sym{*}  &       0.157         &      0.0733         &      0.0981         &      0.0423         \\
            &     (-0.96)         &     (-0.19)         &     (-0.26)         &      (0.54)         &     (-1.80)         &      (2.06)         &      (0.80)         &     (-1.92)         &      (0.86)         &     (-1.23)         &      (7.29)         &     (-1.31)         &     (-2.15)         &      (1.51)         &      (0.99)         &      (1.45)         &      (1.12)         \\
[1em]
Model       &       0.153         &     0.00329         &       0.410\sym{**} &     -0.0169         &      -0.126         &       0.120         &       0.397\sym{***}&     -0.0283         &     -0.0113         &     -0.0724         &       0.167         &      -0.143         &       0.111         &       0.143         &      0.0906         &      0.0766         &     -0.0886         \\
            &      (1.19)         &      (0.08)         &      (3.16)         &     (-0.15)         &     (-1.19)         &      (1.05)         &      (3.49)         &     (-0.27)         &     (-0.15)         &     (-1.19)         &      (1.45)         &     (-1.30)         &      (0.66)         &      (0.83)         &      (0.74)         &      (0.66)         &     (-1.34)         \\
[1em]
Fiscal      &       0.128         &     -0.0211         &      0.0697         &     -0.0468         &       0.117         &       0.255\sym{**} &      0.0550         &      -0.122\sym{**} &      0.0325         &     -0.0550         &       0.304         &     -0.0683         &       0.388\sym{*}  &     -0.0371         &      0.0811         &      0.0303         &     -0.0104         \\
            &      (1.82)         &     (-0.73)         &      (0.94)         &     (-0.59)         &      (1.45)         &      (3.21)         &      (0.60)         &     (-2.76)         &      (0.47)         &     (-1.22)         &      (1.44)         &     (-0.98)         &      (2.55)         &     (-0.61)         &      (1.46)         &      (0.54)         &     (-0.21)         \\
[1em]
Productivity&      0.0277         &     -0.0381         &      0.0865         &     -0.0194         &     0.00816         &      0.0199         &       0.118         &     -0.0602         &     0.00750         &      0.0288         &      0.0145         &     -0.0559         &     -0.0806         &     -0.0618         &       0.238         &     -0.0409         &      0.0101         \\
            &      (0.24)         &     (-1.25)         &      (1.02)         &     (-0.20)         &      (0.11)         &      (0.23)         &      (1.27)         &     (-0.91)         &      (0.11)         &      (0.51)         &      (0.15)         &     (-0.78)         &     (-0.87)         &     (-0.56)         &      (1.87)         &     (-0.54)         &      (0.21)         \\
[1em]
Trade       &      0.0363         &     -0.0362         &      0.0259         &     -0.0482         &     -0.0805         &      0.0639         &       0.152         &      0.0710         &   -0.000366         &      -0.109\sym{*}  &    -0.00596         &     -0.0668         &      0.0443         &       0.251         &       0.433\sym{***}&      0.0583         &      -0.107\sym{**} \\
            &      (0.39)         &     (-1.11)         &      (0.26)         &     (-0.70)         &     (-1.14)         &      (0.82)         &      (1.49)         &      (0.91)         &     (-0.01)         &     (-2.37)         &     (-0.06)         &     (-0.67)         &      (0.53)         &      (1.77)         &      (3.64)         &      (0.79)         &     (-2.81)         \\
[1em]
FOMC        &      -0.101         &      0.0484         &      -0.136         &       0.136         &       0.280         &       0.133         &      0.0989         &      0.0524         &      0.0748         &       0.157\sym{*}  &     -0.0410         &      -0.107         &      0.0987         &      0.0804         &       0.281         &      0.0688         &     -0.0226         \\
            &     (-0.84)         &      (0.88)         &     (-0.94)         &      (1.10)         &      (1.85)         &      (1.07)         &      (0.75)         &      (0.62)         &      (0.80)         &      (2.17)         &     (-0.23)         &     (-0.79)         &      (0.65)         &      (0.48)         &      (1.80)         &      (0.60)         &     (-0.30)         \\
[1em]
Deflation   &      0.0401         &      0.0122         &       0.146         &       0.238         &      -0.109         &      -0.216         &     -0.0852         &     -0.0113         &       0.188\sym{*}  &     -0.0514         &      -0.124         &     0.00563         &       0.110         &      0.0458         &      -0.223\sym{*}  &       0.145         &       0.622\sym{***}\\
            &      (0.39)         &      (0.15)         &      (1.66)         &      (1.56)         &     (-0.76)         &     (-1.88)         &     (-0.76)         &     (-0.13)         &      (2.04)         &     (-0.83)         &     (-1.06)         &      (0.07)         &      (0.68)         &      (0.41)         &     (-2.16)         &      (1.58)         &      (8.48)         \\
[1em]
Constants   &      0.0297         &      0.0113         &    -0.00196         &      0.0108         &      0.0131         &     0.00935         &     0.00982         &      0.0595\sym{***}&    0.000641         &      0.0304\sym{*}  &      0.0142         &      0.0503\sym{**} &     -0.0180         &    -0.00470         &    -0.00457         &     -0.0229         &      0.0211\sym{*}  \\
            &      (1.47)         &      (1.37)         &     (-0.10)         &      (0.53)         &      (0.82)         &      (0.60)         &      (0.49)         &      (4.13)         &      (0.06)         &      (2.23)         &      (0.78)         &      (3.18)         &     (-0.85)         &     (-0.17)         &     (-0.24)         &     (-1.33)         &      (2.01)         \\
\hline
\(N\)       &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         &          95         \\
\hline\hline
\multicolumn{18}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{18}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> var_q_no_control_mod.tex <==
% In order to make the table nice after it has been outputted from Stata:
% 1. Add the following to the second header:
%\multicolumn{1}{c}{\shortstack{Model $\rightarrow$\\Lagged variables (1 lag) $\downarrow$}}
% 2. Change the tabular to:
%       \begin{tabular}{l a b a b a b a b a b a}
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l a b a b a b a b a b a b a b a b a b a b a b a b a b a b a}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\multicolumn{1}{c}{\shortstack{Model $\rightarrow$\\Lagged variables (1 lag) $\downarrow$}}
            &\multicolumn{1}{c}{Housing}&\multicolumn{1}{c}{Regulation}&\multicolumn{1}{c}{\shortstack{Financial\\markets}}&\multicolumn{1}{c}{Trade}&\multicolumn{1}{c}{Purchase}\\
\hline
Housing     &       0.733\sym{***}&    -0.00755         &       0.277\sym{*}  &     -0.0329         &       0.231\sym{**} \\
            &      (8.47)         &     (-0.07)         &      (2.28)         &     (-0.55)         &      (3.05)         \\
[1em]
Regulation  &     -0.0271         &       0.414\sym{***}&      0.0696         &      -0.125\sym{*}  &       0.136\sym{*}  \\
            &     (-0.39)         &      (4.02)         &      (0.86)         &     (-2.11)         &      (2.30)         \\
[1em]
\shortstack{Financial\\markets}&       0.100         &       0.129         &       0.175         &       0.148         &      0.0499         \\
            &      (0.95)         &      (0.80)         &      (1.42)         &      (1.56)         &      (0.44)         \\
[1em]
Trade       &      0.0517         &     -0.0389         &       0.122         &       0.160         &      -0.123         \\
            &      (0.62)         &     (-0.40)         &      (1.00)         &      (1.79)         &     (-1.35)         \\
[1em]
Purchase    &     -0.0165         &       0.296\sym{*}  &       0.132         &      -0.198\sym{***}&       0.557\sym{***}\\
            &     (-0.23)         &      (2.32)         &      (1.53)         &     (-3.75)         &      (7.71)         \\
[1em]
Constants   &     0.00338         &      0.0152         &      0.0335\sym{***}&      0.0487\sym{***}&     0.00920         \\
            &      (0.46)         &      (1.34)         &      (3.41)         &      (4.75)         &      (0.71)         \\
\hline
\(N\)       &          95         &          95         &          95         &          95         &          95         \\
\hline\hline
\multicolumn{6}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{6}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}

